Graph-Controlled Insertion-Deletion Systems

In this article, we consider the operations of insertion and deletion working in a graph-controlled manner. We show that like in the case of context-free productions, the computational power is strictly increased when using a control graph: computational completeness can be obtained by systems with insertion or deletion rules involving at most two symbols in a contextual or in a context-free manner and with the control graph having only four nodes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{88}
\providecommand{\publicationstatus}{I. McQuillan and G. Pighizzini (Eds.): 12th International Workshop\\on Descriptional Complexity of Formal Systems (DCFS 2010)\\
EPTCS 31, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.31.11}{10.4204/EPTCS.31.11}}

